A Hierarchical Approach to Remote Sensing Scene Classification

Remote sensing scene classification deals with the problem of classifying land use/cover of a region from images. To predict the development and socioeconomic structures of cities, the status of land use in regions is tracked by the national mapping agencies of countries. Many of these agencies use land-use types that are arranged in multiple levels. In this paper, we examined the efficiency of a hierarchically designed Convolutional Neural Network (CNN) based framework that is suitable for such arrangements. We use the NWPU-RESISC45 dataset for our experiments and arranged this data set in a two-level nested hierarchy. Each node in the designed hierarchy is trained using DenseNet-121 architectures. We provide detailed empirical analysis to compare the performances of this hierarchical scheme and its non-hierarchical counterpart, together with the individual model performances. We also evaluated the performance of the hierarchical structure statistically to validate the presented empirical results. The results of our experiments show that although individual classifiers for different sub-categories in the hierarchical scheme perform considerably well, the accumulation of the classification errors in the cascaded structure prevents its classification performance from exceeding that of the non-hierarchical deep model

==> MyNotes.tex <==
\section{ResponSeNotes}
\label{sec:51}

\textcolor{red}{Hiyerarşik yapı çalışırken,kullanılan kod imgeleri tek tek alıp tahmin etmek üzerine kurulu. İmgeyi diskten okunduktan sonra ilk sınıflandırıcıya gidiyor. Burada birinci seviye sınıflara  ayrıldıktan sonra if ve switch case ifadeleri kullanılarak ayrıntı sınıfları için tekrar sınıflandırılıyor.

Ölçüm yaparken; konvolüsyonel modellerin ve I/O işleminin süreyi domine etmesi dikkate alınmıştır. Bu sebeple Keras ImageGenerator sınıfı kullanılarak batch hazırlanmıştır.  Modellerin tümü özdeş olduğu için, ImageGenerator Eval fonksiyonu giriş ve çıkışı arasındaki zaman ölçülmüştür.  Eval fonksiyonu çıkışında ImageGenerator ile oluşturulmuş olan batch doğrudan ikinci modele gönderilmiş ve burada Eval fonksiyonu tekrar çalıştırılmıştır.  Eval fonksiyomu çıkışında alınan zaman iki modelin peşpeşe çalıştığı toplam zamanı vermektedir. İlk modelin tek başına çalışması ile de Basix Classifier süreleri hesaplanmıştır.} 

